ttbar production cross section in ppbar collisions at sqrt{s} = 1.8 TeV

Results are presented on a measurement of the ttbar pair production cross section in ppbar collisions at sqrt{s} = 1.8 TeV from nine independent decay channels. The data were collected by the Dzero experiment during the 1992-1996 run of the Fermilab Tevatron Collider. A total of 80 candidate events are observed with an expected background of 38.8 +- 3.3 events. For a top quark mass of 172.1 GeV/c^2, the measured cross section is 5.69 +- 1.21 (stat) +- 1.04 (sys) pb.

==> list_of_visitor_addresses_r1.tex <==
% list_of_visitor_addresses_r1.tex                            8/31/01
%
%\bibitem[\dag]{name}
\bibitem[*]{lehner}
Also at University of Zurich, Zurich, Switzerland.
\bibitem[\dag]{przybycien}
Also at Institute of Nuclear Physics, Krakow, Poland.
%
\vskip 0.25cm

